Adaptive Shortcut Debiasing for Online Continual Learning

We propose a novel framework DropTop that suppresses the shortcut bias in online continual learning (OCL) while being adaptive to the varying degree of the shortcut bias incurred by continuously changing environment. By the observed high-attention property of the shortcut bias, highly-activated features are considered candidates for debiasing. More importantly, resolving the limitation of the online environment where prior knowledge and auxiliary data are not ready, two novel techniques -- feature map fusion and adaptive intensity shifting -- enable us to automatically determine the appropriate level and proportion of the candidate shortcut features to be dropped. Extensive experiments on five benchmark datasets demonstrate that, when combined with various OCL algorithms, DropTop increases the average accuracy by up to 10.4% and decreases the forgetting by up to 63.2%.

==> figures/ablation.tex <==
% \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.}% make the row margin compact
\begin{table}[t]
% \small
\scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
\caption{Ablation study on multi-level feature fusion and drop intensity shifting with respect to $A_{avg}$ on Split CIFAR-100. The highest values are marked in bold. }
\vspace*{-0.3cm}
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
% {@{}c|c||C{0.9cm}C{1.1cm}||C{0.9cm}c@{}}
% {@{}c||C{1.1cm}|C{1.2cm}|C{1.2cm}|C{1.1cm}c@{}}
{@{}l||c|c|c|cc@{}}
\toprule
% \multicolumn{1}{c||}{} & \multicolumn{3}{c|}{\textbf{{    Variants   }}} & \multicolumn{1}{c}{} \\\cline{2-4}
\multicolumn{1}{c||}{\textbf{}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{No Drop Int. Shift}} & \multicolumn{1}{c}{} \\
% \smallskip
\multicolumn{1}{c||}{\hspace{-0.3cm}\textbf{Method}} %\textbf{Method}}
& \multicolumn{1}{c|}{\textbf{No MF}\hspace{-1cm}}
& \multicolumn{1}{c|}{\textbf{Rand Drop}}
& \multicolumn{1}{c|}{\textbf{Top Drop}}
& \multicolumn{1}{c}{\textbf{SDOCL}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c}{\bm{$A_{avg}$}}

\\ \toprule
% seq-cifar100---gss---adl_qty_spatialrdl_greedygreedy_10_0.05_0.9_init_0.1_0.0_evalperiod3---drop_thrh0.95_select_drop_prob1.0_gating_pos4_mean_accs_classil.csv
% & \begin{tabular}[c]{@{}c@{}}{ {19.98}\,($\pm$0.14) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {22.22}\,($\pm$0.53) }\end{tabular}

% seq-cifar100---mir---adl_qty_spatialrdl_greedygreedy_10_0.05_0.9_evalperiod3---drop_thrh0.95_select_drop_prob1.0_gating_pos4_mean_accs_classil.csv
% & \begin{tabular}[c]{@{}c@{}}{ {21.9}\,($\pm$0.24) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {27.4}\,($\pm$0.74) }\end{tabular}

% seq-cifar100---aser---adl_qty_spatialrdl_greedygreedy_10_0.05_0.9_init_0.1_0.0_evalperiod3---drop_thrh0.95_select_drop_prob1.0_gating_pos4_mean_accs_classil.csv
% & \begin{tabular}[c]{@{}c@{}}{ {30.62}\,($\pm$0.31) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {37.82}\,($\pm$0.55) }\end{tabular}

% seq-cifar100---er---adl_qty_spatialrdl_greedygreedy_10_0.05_0.9_evalperiod3---drop_thrh0.95_select_drop_prob1.0_gating_pos4_mean_accs_classil.csv
% & \begin{tabular}[c]{@{}c@{}}{ {26.17}\,($\pm$0.15) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {18.82}\,($\pm$0.18) }\end{tabular}

% seq-cifar100---derpp---adl_qty_spatialrdl_greedygreedy_10_0.05_0.9_evalperiod3---drop_thrh0.95_select_drop_prob1.0_gating_pos4_mean_accs_classil.csv
% & \begin{tabular}[c]{@{}c@{}}{ {23.36}\,($\pm$0.27) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {29.13}\,($\pm$0.39) }\end{tabular}
% # ER ###############################################################
\multirow{1}{*}{ER~\cite{rolnick2019experience}\hspace{-0.15cm}}                                
& \begin{tabular}[c]{@{}c@{}}{{26.2}\,($\pm$0.2)\hspace{-1cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{25.5}\,($\pm$0.3)}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{25.5}\,($\pm$0.2)}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\textbf{{ 26.5 }}\,($\pm$0.2)}\end{tabular}
\\
% \midrule
% \cdashline{}
% # ER ###############################################################


% DER ++ ###############################################################
\multirow{1}{*}{DER++~\cite{buzzega2020dark}\hspace{-0.15cm}}                                                   
& \begin{tabular}[c]{@{}c@{}}{{23.4}\,($\pm$0.3)\hspace{-1cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{22.0}\,($\pm$0.2)}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{24.2}\,($\pm$0.3)}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\textbf{{ 25.1 }}\,($\pm$0.3)}\end{tabular}
\\
% \midrule
% % # ++ ###############################################################

% # MIR ################################################################
\multirow{1}{*}{MIR~\cite{mir}\hspace{-0.15cm}}                                               
& \begin{tabular}[c]{@{}c@{}}{{21.9}\,($\pm$0.2)\hspace{-1cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{22.5}\,($\pm$0.7)}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{22.4}\,($\pm$0.3)}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{22.4}\,($\pm$0.1)}\end{tabular}
\\

% # GSS ################################################################
\multirow{1}{*}{GSS~\cite{aljundi2019gradient}\hspace{-0.15cm}}                                 
& \begin{tabular}[c]{@{}c@{}}{{20.0}\,($\pm$0.1)\hspace{-1cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{20.7}\,($\pm$0.2)}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{22.7}\,($\pm$0.3)}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\textbf{{23.7}}\,($\pm$0.2)}\end{tabular}
\\
% \midrule

% # ASER ################################################################
\multirow{1}{*}{ASER~\cite{shim2021online}\hspace{-0.15cm}}                                               
& \begin{tabular}[c]{@{}c@{}}{{30.6}\,($\pm$0.3)\hspace{-1cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\textbf{{34.2}}\,($\pm$0.1)}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{31.8}\,($\pm$0.2)}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{33.4}\,($\pm$0.4)}\end{tabular}
\\
\midrule
% \cdashline{}


\multirow{1}{*}{\textbf{AVG}\,\textbf{(Degrad.)}\hspace{-0.15cm}}                                               
% # AVG ################################################################
& \begin{tabular}[c]{@{}c@{}}{{24.4}\,(\textbf{-7.4\%})\hspace{-1cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{25.0}\,(\textbf{-4.8\%})}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{{25.3}\,(\textbf{-3.6\%})}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\textbf{{26.2}}}\end{tabular}
% \\
% \multirow{1}{*}{\textbf{Degrad}}                                               
% & \begin{tabular}[c]{@{}c@{}}{ {24.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {25.3} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {25.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{{26.2}} }\end{tabular}
\\
\bottomrule
\end{tabular}
\label{tbl:ablation}

\end{table}


==> figures/algorithm.tex <==

% \algsetup{linenosize=\small}\newlength{\oldtextfloatsep}\setlength{\oldtextfloatsep}{\textfloatsep}
\setlength{\textfloatsep}{10pt}% Remove \textfloatsep
\begin{algorithm}[!t]
% \small
\footnotesize
\caption{\small Replay-based OCL with \algname{}}
\label{alg:pseudocode}
\begin{algorithmic}[1]
\REQUIRE {Number of tasks $T$, online data stream $\{D_1,\dots,D_T\}$, total drop rate $\gamma$, softmax function $\sigma$, learning rate $\eta$, batch size $b$
% \\
% economy-view $X_{\mathcal{B}}$, geography-view $X_{\mathcal{G}}$, epidemic-view $X_{\mathcal{P}}$, \\
% economic impact trend $\mathbb{Y}$
}
\ENSURE {Model parameters $\theta, w$ after learning task $T$}
\STATE {$\theta, w \leftarrow \text{Initialize model parameters};$}
\label{lst:line:init_s}
\STATE {$\mathcal{B} \leftarrow \text{Initialize replay memory};$}
\STATE {$\kappa \leftarrow \text{Initialize class-wise debiasing intensity};$}
\label{lst:line:init_e}
\FOR {$t=1$ {\bf to} $T$}
\FOR {$i=1$ {\bf to} $|D_t|/b$}
\STATE {${X}_n, {Y}_n$ $\leftarrow$ a mini-batch from online data stream $D_t$;} 
\label{lst:line:online_batch}
\STATE {\COMMENT{\textsc{Replay Memory Retrieval}}}
\STATE {${X}_m, {Y}_m$ $\leftarrow$ ${\rm MemoryRetrieve}(\mathcal{B}, {X}_n, {Y}_n)$;} 
\label{lst:line:memory_batch}
\STATE {\COMMENT{\textbf{\textsc{Attentive Debias Layer in \cref{subsec: Attentive Debiasing Layer}}}}}
\label{lst:line:online_debiasing_layer}
\STATE {$M$ $\leftarrow$ ${\rm MultiLevelDropMask}({X}_n\cup{X}_m;\theta,\kappa,\gamma)$;}\hspace*{-1cm}
\label{lst:line:drop_mask}
\STATE {$P$ $\leftarrow$ $\sigma({\rm DebiasForward}({X}_n\cup{X}_m, M; \theta, w)) $;} 
\label{lst:line:debias_forward}
\STATE {\COMMENT{\textsc{Model Update}}}
\label{lst:line:update_s}
\STATE {Compute the loss $\mathcal{J}$ using ${Y}_n\cup{Y}_m$ and ${P}$;}
\STATE {$\theta \leftarrow \theta - \eta\nabla_{\theta}\mathcal{J}$;$w \leftarrow w - \eta\nabla_{w}\mathcal{J}$;}
% \STATE {$\phi \leftarrow \phi - \eta\nabla_{\phi}\mathcal{J}$;}
\label{lst:line:update_e}
\STATE {\COMMENT{\textsc{Replay Memory Update}}}
\label{lst:line:mem_update_s}
\STATE {$\mathcal{B}$ $\leftarrow$ ${\rm MemoryUpdate}(\mathcal{B}, {X}_n, {Y}_n)$;} 
\label{lst:line:mem_update_e}
\STATE {\COMMENT{\textbf{\textsc{Adjust Drop Intensity in \cref{subsec: Adaptive Debiasing Intensity Scheduler}}}}}
\label{lst:line:adjust_s}
\STATE {$\kappa$ $\leftarrow$ ${\rm AdjustDropIntensity}(\mathcal{M}, i)$;} 
\label{lst:line:adjust_e}
\ENDFOR
\ENDFOR
% \ENDFOR
\RETURN {$\theta^*,w^*$;}
\end{algorithmic}
\end{algorithm}
% \vspace{-0.1cm}

==> figures/algorithm_adaptive_scheduler.tex <==
% \renewcommand\algorithmiccomment[1]{%
%   \hfill\#\ \eqparbox{COMMENT}{#1}%
% }

\algsetup{linenosize=\footnotesize}\newlength{\oldtextfloatsep}\setlength{\oldtextfloatsep}{\textfloatsep}
\setlength{\textfloatsep}{8pt}% Remove \textfloatsep
\begin{algorithm}[!t]
% \small

\caption{\small Adaptive Intensity Shifting}
\label{alg:pseudocode_adaptive_scheduler}
\begin{algorithmic}[1]
\footnotesize 
\REQUIRE {Preceding intensity: $\kappa^\prime$, step size: $\alpha$, alternating period: $p$, episodic memory of each class: $\mathcal{B}$, model parameters: $\{\theta,w\}$, training iteration: $i$
% \\
% economy-view $X_{\mathcal{B}}$, geography-view $X_{\mathcal{G}}$, epidemic-view $X_{\mathcal{P}}$, \\
% economic impact trend $\mathbb{Y}$
}
\ENSURE {Drop intensity $\kappa$ that will be applied to the next model update}
\STATE {\COMMENT{{\textsc{Initialize candidate strategies}}}}
\STATE {$\kappa^{dec} \leftarrow \kappa^\prime*\alpha; ~~\kappa^{inc} \leftarrow \kappa^\prime * (1/\alpha);$}
\STATE {\{$\mathcal{H}^{dec}, \mathcal{H}^{inc}\} \leftarrow {\rm InitializeHistory}()$;}
\IF{${\rm mod}(i,p)=0$} 
% \COMMENT{Compute Contribution of Intensity}
\STATE {\COMMENT{{\textsc{Compute contribution of intensity}}}}
% \STATE {$\mathcal{J}_{new}$ $\leftarrow$ ${\rm Loss}(\mathcal{B}, \{\theta_i, w_i\})$;~~ $\Delta\mathcal{J}\leftarrow \mathcal{J}_{old}-\mathcal{J}_{new}$;} 
\STATE {$\mathcal{L}_{new}$ $\leftarrow$ ${\rm Loss}(\mathcal{B}, \{\theta, w\})$;}
\STATE {$\Delta\mathcal{L}\leftarrow \mathcal{L}_{old}-\mathcal{L}_{new}$;} 
% \label{lst:line:online_batch}
\STATE { ${\rm UpdateHistory}(\{\mathcal{H}^{dec}, \mathcal{H}^{inc}\}, \Delta\mathcal{L})$;} 
\STATE {$\mathcal{L}_{old}$ $\leftarrow$ $\mathcal{L}_{new}$;} 
\STATE {\COMMENT{{\textsc{Update Intensity based on Statistical Test}}}}
\IF {${\rm full}(\mathcal{H}^{dec}, \mathcal{H}^{inc})$}
\IF {${\rm \textit{p}\text{-}value}(\mathcal{H}^{dec}, \mathcal{H}^{inc})\le0.05$}
    \STATE {$\kappa^{inc}$ $\leftarrow$ $\kappa^{dec}$;}
    \STATE {$\kappa^{dec}$ $\leftarrow$ $\kappa^{dec}*\alpha$;}
\ELSIF{${\rm \textit{p}\text{-}value}(\mathcal{H}^{dec}, \mathcal{H}^{inc})\ge0.95$}
    \STATE {$\kappa^{dec}$ $\leftarrow$ $\kappa^{inc}$;}
    \STATE {$\kappa^{inc}$ $\leftarrow$ $\kappa^{inc}*(1/\alpha)$;}
\ENDIF
\STATE {${\rm ResetHistory}(\mathcal{H}^{dec}, \mathcal{H}^{inc})$;}
\ENDIF
\STATE {\COMMENT{{\textsc{Alternate two shift directions} }}}
\STATE {$\kappa \leftarrow {\rm AlternateBetween}(\kappa^{dec}, \kappa^{inc},i)$ ;} 
% \RETURN {$\kappa$;}
%%%%%%% Details of AlternateIntensity() %%%%%%%%
% \IF {$div(i,2)=0$}
%     \STATE {$\kappa \leftarrow \kappa^{dec}$;}    
%     \RETURN {$\kappa$;}
% \ELSE
%     \STATE {$\kappa \leftarrow \kappa^{inc}$;}    
%     \RETURN {$\kappa$;}
% \ENDIF
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ELSE 
% \COMMENT{{\textsc{Keep Applying Current Intensity}}}
\STATE {$\kappa \leftarrow \kappa^\prime$;} 
\ENDIF
\RETURN {$\kappa$;}
\end{algorithmic}
\end{algorithm}


==> figures/overall_performance.tex <==
% \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.0}% make the row margin compact
\begin{table*}[t]
% \small
\scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
\caption{Performance comparisons on CIFAR10, CIFAR100, and SuperImageNet-9 for biased setup. The highest values are marked in bold. The mean of \emph{five} repetitions with different random initialization were reported. }
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
{@{}c|c||cc|cc|cc|cc|ccc@{}}
% {@{}c|c|ccccccccc@{}}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{1}{c||}{} & \multicolumn{6}{c|}{\textbf{\underline{    Biased Setup    }}} & \multicolumn{4}{c}{\textbf{\underline{    Unbiased Setup   }}} \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c||}{} & \multicolumn{2}{c}{\textbf{CIFAR10}} & \multicolumn{2}{c}{\textbf{CIFAR100}} & \multicolumn{2}{c|}{\textbf{IN-9}} & \multicolumn{2}{c}{\textbf{IN-OnlyFG}} & \multicolumn{2}{c}{\textbf{IN-Stylized}} \\
% \smallskip
\multicolumn{1}{c|}{\textbf{Method}}
& \multicolumn{1}{c||}{\textbf{Debias Method}}
& \multicolumn{1}{c}{\bm{$F_{last}$}}
& \multicolumn{1}{c|}{\bm{$A_{avg}$}}
& \multicolumn{1}{c}{\bm{$F_{last}$}}
& \multicolumn{1}{c|}{\bm{$A_{avg}$}}
& \multicolumn{1}{c}{\bm{$F_{last}$}}
& \multicolumn{1}{c|}{\bm{$A_{avg}$}}
& \multicolumn{1}{c}{\bm{$F_{last}$}}
& \multicolumn{1}{c|}{\bm{$A_{avg}$}}
& \multicolumn{1}{c}{\bm{$F_{last}$}}
& \multicolumn{1}{c}{\bm{$A_{avg}$}}


\\ \toprule
% # ER ###############################################################
\multirow{2}{*}{ER}                                
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 39.89 }\,($\pm$2.35) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 55.36 }\,($\pm$0.30) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 19.22 }\,($\pm$0.25) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 25.34 }\,($\pm$0.18) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {50.95}\,($\pm$2.14) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {44.48}\,($\pm$1.38) }\end{tabular}

& \begin{tabular}[c]{@{}c@{}}{ 17.6 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 29.1 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{40.3} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 37.60 }\,($\pm$1.89) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 61.02 }\,($\pm$0.61) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 18.28 }\,($\pm$1.31) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 26.45 }\,($\pm$0.17) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {36.12}\,($\pm$4.74) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {48.94}\,($\pm$1.01) }\end{tabular}

& \begin{tabular}[c]{@{}c@{}}{ \textbf{19.2} ($\pm$ 0.12) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 28.7 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{29.8} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 39.4 }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{59.9} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{23.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{24.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 32.4 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{45.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 15.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{30.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 26.7 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 39.5 }\end{tabular}
\\
\midrule
% # ER ###############################################################


% DER ++ ###############################################################
\multirow{2}{*}{DER++}                                                         
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 28.20 }\,($\pm$1.48) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 59.76 }\,($\pm$0.76) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 33.43 }\,($\pm$0.73) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 23.64 }\,($\pm$0.32) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {63.0}\,($\pm$4.62) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {44.2}\,($\pm$1.01) }\end{tabular}

& \begin{tabular}[c]{@{}c@{}}{ 12.3 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 28.2 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 22.7 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 37.9 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 23.68 }\,($\pm$0.98) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 62.56 }\,($\pm$0.73) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 31.11 }\,($\pm$1.15) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 25.14 }\,($\pm$0.27) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {60.73}\,($\pm$5.06) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {45.42}\,($\pm$0.54) }\end{tabular}

& \begin{tabular}[c]{@{}c@{}}{ \textbf{13.8} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{29.5} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{23.5} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{38.9} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{51.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{61.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{21.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 23.2 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{30.6 }}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{43.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{19.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{29.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{26.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{38.5} }\end{tabular}
\\
\midrule
% % # ++ ###############################################################

% # MIR ################################################################
\multirow{2}{*}{MIR}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {58.42}\,($\pm$1.28) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {51.54}\,($\pm$0.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {25.32}\,($\pm$1.69) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {20.75}\,($\pm$0.56) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.07}\,($\pm$1.99) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.34}\,($\pm$1.18) }\end{tabular}

& \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {56.25}\,($\pm$1.58) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {51.63}\,($\pm$0.56) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {25.06}\,($\pm$1.05) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {21.72}\,($\pm$0.34) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.25}\,($\pm$4.47) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {42.01}\,($\pm$0.93) }\end{tabular}

& \begin{tabular}[c]{@{}c@{}}{ \textbf{18.9} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{36.5} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{39.4}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{50.7} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{62.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{69.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 35.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{31.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{52.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{56.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{20.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{33.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\textbf{39.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
\\
\midrule


% # GSS ################################################################
\multirow{2}{*}{GSS}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {69.66}\,($\pm$0.71) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {46.04}\,($\pm$0.42) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {24.22}\,($\pm$0.73) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {20.95}\,($\pm$0.37) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {71.53}\,($\pm$2.01) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {40.33}\,($\pm$0.63) }\end{tabular}

& \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {69.22}\,($\pm$1.53) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {49.05}\,($\pm$0.46) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {29.06}\,($\pm$0.87) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {24.45}\,($\pm$0.27) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {68.53}\,($\pm$1.87) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.26}\,($\pm$0.57) }\end{tabular}

& \begin{tabular}[c]{@{}c@{}}{ \textbf{18.9} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{36.5} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{39.4}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{50.7} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{62.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{69.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 35.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{31.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{52.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{56.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{20.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{33.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\textbf{39.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
\\
\midrule

% # ASER ################################################################
\multirow{2}{*}{ASER}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 57.77 }\,($\pm$3.33) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 50.32 }\,($\pm$0.45) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 41.77 }\,($\pm$0.41) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 32.68 }\,($\pm$0.10) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {62.63}\,($\pm$2.05) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.7}\,($\pm$0.72) }\end{tabular}

& \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 57.54 }\,($\pm$0.75) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 51.32 }\,($\pm$0.32) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 39.54 }\,($\pm$0.81) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ { 33.43 }\,($\pm$0.38) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {57.5}\,($\pm$3.18) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.6}\,($\pm$0.76) }\end{tabular}

& \begin{tabular}[c]{@{}c@{}}{ \textbf{18.9} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{36.5} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{39.4}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{50.7} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{62.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{69.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 35.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{31.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{52.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{56.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{20.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{33.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\textbf{39.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
\\
\bottomrule



% \midrule
% # TADA ################################################################

% % # DEFSI ###############################################################
% \multirow{3}{*}{DEFSI}                                              
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Jung }\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.23 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 1.04 }\,($\pm$0.01)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.34 }\,($\pm$0.04)\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}{ 0.64 }\,($\pm$0.02)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.38 }\,($\pm$0.08)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.22 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 1.15 }\,($\pm$0.05)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\hspace*{-0.2cm}{ 0.32 }\,($\pm$0.06)\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Jungnang }\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}{ 0.51 }\,($\pm$0.02)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.51 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.17 }\,($\pm$0.01)\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.25 }\,($\pm$0.00)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.21 }\,($\pm$0.02)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.36 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.42 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\hspace*{-0.2cm}{ 0.27 }\,($\pm$0.02)\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Mapo }\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}{ 0.28 }\,($\pm$0.04)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.52 }\,($\pm$0.04)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.29 }\,($\pm$0.01)\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}{ 0.63 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.61 }\,($\pm$0.05)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.32 }\,($\pm$0.04)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.66 }\,($\pm$0.04)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\hspace*{-0.2cm}{ 0.55 }\,($\pm$0.06)\end{tabular}
% \\
% \midrule
% % # DEFSI ###############################################################


% % # OURS ###############################################################
% \multirow{3}{*}{\textbf{\algname{}}}
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Jung }\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}{ 0.30 }\,($\pm$0.04)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 1.01 }\,($\pm$0.01)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.16 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.32 }\,($\pm$0.04)\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.14 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.22 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.78 }\,($\pm$0.04)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\hspace*{-0.2cm}\textbf{ 0.22 }\,($\pm$0.03)\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Jungnang }\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.33 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.35 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 0.41 }\,($\pm$0.03)\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}{ 0.26 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.17 }\,($\pm$0.01)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.23 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.25 }\,($\pm$0.02)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\hspace*{-0.2cm}\textbf{ 0.25 }\,($\pm$0.02)\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Mapo }\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.20 }\,($\pm$0.04)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.28 }\,($\pm$0.02)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.19 }\,($\pm$0.04)\end{tabular}
% % & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.32 }\,($\pm$0.05)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.56 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.26 }\,($\pm$0.03)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\textbf{ 0.34 }\,($\pm$0.06)\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}\hspace*{-0.2cm}\textbf{ 0.27 }\,($\pm$0.03)\end{tabular}
% # OURS ###############################################################

\end{tabular}
\label{tbl:overall_comparison_biased_setup}
\end{table*}


==> figures/performance_biased_setup.tex <==
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.0}% make the row margin compact
\begin{table*}[t]
\small
\scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
\caption{Average accuracy\,(higher is better) and forgetting\,(lower is better) on Split CIFAR-100, Split CIFAR-10, and Split ImageNet-9 for biased setup\,(The best results are marked in bold). The mean of \emph{five} repetitions with different random initialization were reported. }
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
{@{}l|c||C{1.85cm}c|C{1.85cm}c|C{1.85cm}cc@{}}
% {@{}c|c|ccccccccc@{}}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{1}{c||}{} & \multicolumn{6}{c}{\textbf{\underline{    Biased Setup    }}} \\
% & \multicolumn{4}{c}{\textbf{{    Unbiased Setup   }}} \\
\multicolumn{1}{c|}{\textbf{OCL}} & \multicolumn{1}{c||}{\textbf{Debias}} & \multicolumn{2}{c}{\textbf{Split CIFAR-100}} & \multicolumn{2}{c}{\textbf{Split CIFAR-10}} & \multicolumn{2}{c}{\textbf{Split ImageNet-9}} \\
% & \multicolumn{2}{c}{\textbf{IN-OnlyFG}} & \multicolumn{2}{c}{\textbf{IN-Stylized}} \\
% \smallskip
\multicolumn{1}{c|}{\textbf{Method}}
& \multicolumn{1}{c||}{\textbf{Method}}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c|}{\bm{$F_{last}$}\,($\downarrow$)}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c|}{\bm{$F_{last}$}\,($\downarrow$)}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c}{\bm{$F_{last}$}\,($\downarrow$)}
% & \multicolumn{1}{c}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c|}{\bm{$F_{last}$}}
% & \multicolumn{1}{c}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
\\ \toprule
% # ER ###############################################################
\multirow{2}{*}{ER~\cite{rolnick2019experience}}                                
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {25.34}\,($\pm$0.18) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {19.22}\,($\pm$0.25) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {55.36}\,($\pm$0.30) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.89}\,($\pm$2.35) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {46.05}\,($\pm$0.20) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {55.80}\,($\pm$1.82) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 17.6 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 29.1 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{40.3} }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{26.45}\,($\pm$0.17) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{18.28}\,($\pm$1.31) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{61.02}\,($\pm$0.61) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{37.60}\,($\pm$1.89) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{48.86}\,($\pm$0.43) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{44.01}\,($\pm$3.76) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{19.2} ($\pm$ 0.12) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.7 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{29.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 39.4 }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{59.9} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{23.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{24.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 32.4 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{45.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 15.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{30.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 26.7 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 39.5 }\end{tabular}
\\
\midrule
% # ER ###############################################################

% DER ++ ###############################################################
\multirow{2}{*}{DER++~\cite{buzzega2020dark}}                                                         
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {23.64}\,($\pm$0.32) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {33.43}\,($\pm$0.73) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {59.76}\,($\pm$0.76) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {28.20}\,($\pm$1.48) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {44.20}\,($\pm$1.01) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {63.00}\,($\pm$4.62) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 12.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.2 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 22.7 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.9 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{25.14}\,($\pm$0.27) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{31.11}\,($\pm$1.15) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{62.56}\,($\pm$0.73) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{23.68}\,($\pm$0.98) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{45.42}\,($\pm$0.54) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{60.73}\,($\pm$5.06) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{13.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{29.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{23.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{38.9} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{51.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{61.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{21.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 23.2 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{30.6 }}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{43.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{19.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{29.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{26.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{38.5} }\end{tabular}
\\
\midrule
% % # ++ ###############################################################

% # MIR ################################################################
\multirow{2}{*}{MIR~\cite{mir}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {20.75}\,($\pm$0.56) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {25.32}\,($\pm$1.69) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {51.54}\,($\pm$0.50) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {58.42}\,($\pm$1.28) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.34}\,($\pm$1.18) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.07}\,($\pm$1.99) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{22.44}\,($\pm$0.13) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{24.83}\,($\pm$1.04) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {51.63}\,($\pm$0.56) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{56.25}\,($\pm$1.58) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{42.01}\,($\pm$0.93) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{39.25}\,($\pm$4.47) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ \textbf{18.9} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{36.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{39.4}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.7} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{62.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{69.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 35.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{31.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{52.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{56.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{20.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{33.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\textbf{39.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
\\
\midrule


% # GSS ################################################################
\multirow{2}{*}{GSS~\cite{aljundi2019gradient}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {21.77}\,($\pm$0.34) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {27.94}\,($\pm$0.80) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {46.04}\,($\pm$0.42) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {69.66}\,($\pm$0.71) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {40.33}\,($\pm$0.63) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {71.53}\,($\pm$2.01) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{23.69}\,($\pm$0.16) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{28.41}\,($\pm$1.00) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{49.05}\,($\pm$0.46) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{69.22}\,($\pm$1.53) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{41.26}\,($\pm$0.57) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{68.53}\,($\pm$1.87) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ \textbf{18.9} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{36.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{39.4}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.7} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{62.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{69.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 35.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{31.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{52.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{56.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{20.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{33.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\textbf{39.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
\\
\midrule

% # ASER ################################################################
\multirow{2}{*}{ASER~\cite{shim2021online}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {32.68}\,($\pm$0.10) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.77}\,($\pm$0.41) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {50.32}\,($\pm$0.45) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {57.77}\,($\pm$3.33) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.70}\,($\pm$0.72) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {62.63}\,($\pm$2.05) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{33.43}\,($\pm$0.38) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{39.54}\,($\pm$0.81) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{51.32}\,($\pm$0.32) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{57.54}\,($\pm$0.75) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{41.60}\,($\pm$0.76) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{57.50}\,($\pm$3.18) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ \textbf{18.9} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{36.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{39.4}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.7} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{62.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{69.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 35.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{31.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{52.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{56.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{20.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{33.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\textbf{39.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
\\
\bottomrule


\end{tabular}
}
\label{tbl:overall_comparison_biased_setup}
\end{table*}


==> figures/performance_biased_setup_improv.tex <==
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.0}% make the row margin compact
\begin{table*}[t]
% \small
\scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
\caption{Average accuracy\,(the higher, the better) and forgetting\,(the lower, the better) on Split CIFAR-100, Split CIFAR-10, and Split ImageNet-9 for the biased setup. The highest values are marked in bold. }
% \vspace*{-0.3cm}
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
{@{}l|c||C{1.85cm}c|C{1.85cm}c|C{1.85cm}cc@{}}
% {@{}c|c|ccccccccc@{}}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{1}{c||}{} & \multicolumn{6}{c}{\textbf{\underline{    Biased Setup    }}} \\
% & \multicolumn{4}{c}{\textbf{{    Unbiased Setup   }}} \\
\multicolumn{1}{c|}{\textbf{OCL}} & \multicolumn{1}{c||}{\textbf{Debias}} & \multicolumn{2}{c}{\textbf{Split CIFAR-100}} & \multicolumn{2}{c}{\textbf{Split CIFAR-10}} & \multicolumn{2}{c}{\textbf{Split ImageNet-9}} \\
% & \multicolumn{2}{c}{\textbf{IN-OnlyFG}} & \multicolumn{2}{c}{\textbf{IN-Stylized}} \\
% \smallskip
\multicolumn{1}{c|}{\textbf{Method}}
& \multicolumn{1}{c||}{\textbf{Method}}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c|}{\bm{$F_{last}$}\,($\downarrow$)}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c|}{\bm{$F_{last}$}\,($\downarrow$)}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c}{\bm{$F_{last}$}\,($\downarrow$)}
% & \multicolumn{1}{c}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c|}{\bm{$F_{last}$}}
% & \multicolumn{1}{c}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
\\ \toprule
% # ER ###############################################################
\multirow{3}{*}{ER~\cite{rolnick2019experience}}                                
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {25.34}\,($\pm$0.18) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {19.22}\,($\pm$0.25) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {55.36}\,($\pm$0.30) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.89}\,($\pm$2.35) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {46.05}\,($\pm$0.20) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {55.80}\,($\pm$1.82) }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ \algname{} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{26.45}\,($\pm$0.17) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{18.28}\,($\pm$1.31) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{61.02}\,($\pm$0.61) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{37.60}\,($\pm$1.89) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{48.86}\,($\pm$0.43) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{44.01}\,($\pm$3.76) }\end{tabular}
\\
\addlinespace[0.15ex]\cline{2-8}\addlinespace[0.6ex]
& \begin{tabular}[c]{@{}c@{}}\textrm{ {Rel. Improv.} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 4.38\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 4.89\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 10.22\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 5.74\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 6.11\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 21.13\% }\end{tabular}
\\
\midrule
% # ER ###############################################################

% DER ++ ###############################################################
\multirow{3}{*}{DER++~\cite{buzzega2020dark}}                                                         
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {23.64}\,($\pm$0.32) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {33.43}\,($\pm$0.73) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {59.76}\,($\pm$0.76) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {28.20}\,($\pm$1.48) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {44.20}\,($\pm$1.01) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {63.00}\,($\pm$4.62) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 12.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.2 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 22.7 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.9 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ \algname{} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{25.14}\,($\pm$0.27) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{31.11}\,($\pm$1.15) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{62.56}\,($\pm$0.73) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{23.68}\,($\pm$0.98) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{45.42}\,($\pm$0.54) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{60.73}\,($\pm$5.06) }\end{tabular}
\\
\addlinespace[0.15ex]\cline{2-8}\addlinespace[0.6ex]
& \begin{tabular}[c]{@{}c@{}}\textrm{ {Rel. Improv}. }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 6.35\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 6.94\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 4.69\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 16.03\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 2.76\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 3.60\% }\end{tabular}
\\
\midrule
% % # ++ ###############################################################

% # MIR ################################################################
\multirow{3}{*}{MIR~\cite{mir}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {20.75}\,($\pm$0.56) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {25.32}\,($\pm$1.69) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {51.54}\,($\pm$0.50) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {58.42}\,($\pm$1.28) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.34}\,($\pm$1.18) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.07}\,($\pm$1.99) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ \algname{} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{22.44}\,($\pm$0.13) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{24.83}\,($\pm$1.04) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{51.63}\,($\pm$0.56) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{56.25}\,($\pm$1.58) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{42.01}\,($\pm$0.93) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{39.25}\,($\pm$4.47) }\end{tabular}
\\
\addlinespace[0.15ex]\cline{2-8}\addlinespace[0.6ex]
& \begin{tabular}[c]{@{}c@{}}\textrm{ {Rel. Improv.} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 8.14\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 1.94\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 0.17\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 3.71\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 6.79\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 4.43\% }\end{tabular}
\\
\midrule

% # GSS ################################################################
\multirow{3}{*}{GSS~\cite{aljundi2019gradient}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {21.77}\,($\pm$0.34) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{27.94}\,($\pm$0.80) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {46.04}\,($\pm$0.42) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {69.66}\,($\pm$0.71) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {40.33}\,($\pm$0.63) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {71.53}\,($\pm$2.01) }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ \algname{} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{23.69}\,($\pm$0.16) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {28.41}\,($\pm$1.00) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{49.05}\,($\pm$0.46) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{69.22}\,($\pm$1.53) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{41.26}\,($\pm$0.57) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{68.53}\,($\pm$1.87) }\end{tabular}
\\
\addlinespace[0.15ex]\cline{2-8}\addlinespace[0.6ex]
& \begin{tabular}[c]{@{}c@{}}\textrm{ {Rel. Improv.} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 8.82\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ -1.68\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 6.54\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 0.63\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 2.31\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 4.19\% }\end{tabular}
\\
\midrule

% # ASER ################################################################
\multirow{3}{*}{ASER~\cite{shim2021online}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {32.68}\,($\pm$0.10) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.77}\,($\pm$0.41) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {50.32}\,($\pm$0.45) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {57.77}\,($\pm$3.33) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.70}\,($\pm$0.72) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {62.63}\,($\pm$2.05) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{ \algname{} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{33.43}\,($\pm$0.38) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{39.54}\,($\pm$0.81) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{51.32}\,($\pm$0.32) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{57.54}\,($\pm$0.75) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{41.60}\,($\pm$0.76) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ \textbf{57.50}\,($\pm$3.18) }\end{tabular}
\\
\addlinespace[0.15ex]\cline{2-8}\addlinespace[0.6ex]
& \begin{tabular}[c]{@{}c@{}}\textrm{ {Rel. Improv.} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 2.29\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 5.34\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 1.99\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 0.40\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 4.79\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 8.19\% }\end{tabular}
\\
\bottomrule

\end{tabular}
}
\label{tbl:overall_comparison_biased_setup}
\vspace*{-0.2cm}
\end{table*}


==> figures/performance_biased_unbiased_setup.tex <==
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \bgroup
\def\arraystretch{1.2}% make the row margin compact
\begin{table*}[t]
\small
% \scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
\caption{Average accuracy\,(higher is better) and forgetting\,(lower is better) on Split CIFAR-100, Split CIFAR-10, and Split ImageNet-9 for biased setup and Split ImageNet(IN)-\{OnlyFG, Stylized\} for unbiased setup. The mean of \emph{five} repetitions with different random initialization were reported. }
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
% {@{}c|c||C{1.85cm}c|C{1.85cm}c|C{1.85cm}cc@{}}
{@{}l|ccccccccccc@{}}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{6}{c|}{\textbf{\underline{    Biased Setup    }}} 
& \multicolumn{4}{c}{\textbf{\underline{    Unbiased Setup   }}} \\
% \multicolumn{1}{c|}{\textbf{OCL}} & \multicolumn{1}{c||}{\textbf{Debiasing}} 
\multicolumn{1}{c|}{\textbf{}}& \multicolumn{2}{c}{\textbf{Split CIFAR-100}} & \multicolumn{2}{c}{\textbf{Split CIFAR-10}} & \multicolumn{2}{c|}{\textbf{Split ImageNet-9}}
& \multicolumn{2}{c}{\textbf{Split IN-OnlyFG}} & \multicolumn{2}{c}{\textbf{Split IN-Stylized}} \\
% \smallskip
\multicolumn{1}{c|}{\textbf{Method}}
% & \multicolumn{1}{c||}{\textbf{Method}}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c|}{\bm{$F_{last}$}\,($\downarrow$)}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c|}{\bm{$F_{last}$}\,($\downarrow$)}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c|}{\bm{$F_{last}$}\,($\downarrow$)}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c|}{\bm{$F_{last}$}\,($\downarrow$)}
& \multicolumn{1}{c}{\bm{$A_{avg}$}\,($\uparrow$)}
& \multicolumn{1}{c}{\bm{$F_{last}$}\,($\downarrow$)}
\\ \toprule
% # ER ###############################################################
\multirow{1}{*}{ER~\cite{rolnick2019experience}}                                
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {25.3}\,($\pm$0.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {19.2}\,($\pm$0.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {55.4}\,($\pm$0.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.9}\,($\pm$2.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {46.1}\,($\pm$0.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {55.8}\,($\pm$1.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {32.8}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {45.0}\,($\pm$1.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.3}\,($\pm$0.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {49.7}\,($\pm$0.9) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ 17.6 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 29.1 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{40.3} }\end{tabular}
\\
\multirow{1}{*}{\textbf{~~$+$SDOCL}}  
% & \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {26.5}\,($\pm$0.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {18.3}\,($\pm$1.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {61.0}\,($\pm$0.6) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {37.6}\,($\pm$1.9) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {48.9}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {44.0}\,($\pm$3.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {35.9}\,($\pm$0.9) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {47.8}\,($\pm$3.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.3}\,($\pm$0.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {38.9}\,($\pm$2.6) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{19.2} ($\pm$ 0.12) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.7 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{29.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 39.4 }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{59.9} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{23.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{24.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 32.4 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{45.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 15.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{30.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 26.7 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 39.5 }\end{tabular}
\\
\midrule
% # ER ###############################################################

% DER ++ ###############################################################
\multirow{1}{*}{DER++~\cite{buzzega2020dark}}                                                         
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {23.6}\,($\pm$0.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {33.4}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {59.8}\,($\pm$0.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {28.2}\,($\pm$1.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {44.2}\,($\pm$1.0) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {63.0}\,($\pm$4.6) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {33.2}\,($\pm$0.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {61.6}\,($\pm$2.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {37.8}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {60.3}\,($\pm$3.2) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 12.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.2 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 22.7 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.9 }\end{tabular}
\\
\multirow{1}{*}{\textbf{~~$+$SDOCL}}   
% & \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {25.1}\,($\pm$0.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {31.1}\,($\pm$1.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {62.6}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {23.7}\,($\pm$1.0) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {45.4}\,($\pm$0.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {60.7}\,($\pm$5.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {34.5}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {54.9}\,($\pm$3.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.7}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {58.9}\,($\pm$4.1) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{13.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{29.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{23.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{38.9} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{51.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{61.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{21.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 23.2 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{30.6 }}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{43.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{19.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{29.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{26.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{38.5} }\end{tabular}
\\
\midrule
% % # ++ ###############################################################

% # MIR ################################################################
\multirow{1}{*}{MIR~\cite{mir}}                              

% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {20.8}\,($\pm$0.6) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {25.3}\,($\pm$1.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {51.5}\,($\pm$0.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {58.4}\,($\pm$1.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.3}\,($\pm$1.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.1}\,($\pm$2.0) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {32.1}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {38.9}\,($\pm$3.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {34.0}\,($\pm$1.0) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {40.7}\,($\pm$1.6) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
\multirow{1}{*}{\textbf{~~$+$SDOCL}}
% & \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {22.4}\,($\pm$0.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {24.8}\,($\pm$1.0) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {51.6}\,($\pm$0.6) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {56.3}\,($\pm$1.6) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {42.0}\,($\pm$0.9) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.3}\,($\pm$4.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {35.4}\,($\pm$1.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {36.0}\,($\pm$3.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {36.1}\,($\pm$0.6) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {38.3}\,($\pm$3.4) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ \textbf{18.9} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{36.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{39.4}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.7} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{62.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{69.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 35.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{31.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{52.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{56.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{20.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{33.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\textbf{39.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
\\
\midrule


% # GSS ################################################################
\multirow{1}{*}{GSS~\cite{aljundi2019gradient}}                                               
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {21.8}\,($\pm$0.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {27.9}\,($\pm$0.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {46.0}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {69.7}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {40.3}\,($\pm$0.6) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {71.5}\,($\pm$2.0) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {34.5}\,($\pm$0.9) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {65.6}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {35.3}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {64.2}\,($\pm$1.9) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
\multirow{1}{*}{\textbf{~~$+$SDOCL}}
% & \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {23.7}\,($\pm$0.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {28.4}\,($\pm$1.0) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {49.1}\,($\pm$0.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {69.2}\,($\pm$1.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.3}\,($\pm$0.6) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {68.5}\,($\pm$1.9) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {36.5}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {61.6}\,($\pm$1.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {35.9}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {62.3}\,($\pm$2.3) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ \textbf{18.9} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{36.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{39.4}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.7} }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{ Random }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{62.7} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{69.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 35.0 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{31.1} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{52.4} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{56.5} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{20.0} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{33.6} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\textbf{39.8} }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ \textbf{50.6} }\end{tabular}
\\
\midrule

% # ASER ################################################################
\multirow{1}{*}{ASER~\cite{shim2021online}}                                               
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {32.7}\,($\pm$0.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.8}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {50.3}\,($\pm$0.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {57.8}\,($\pm$3.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.7}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {62.6}\,($\pm$2.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {30.2}\,($\pm$0.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {60.2}\,($\pm$0.9) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {33.6}\,($\pm$0.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {56.8}\,($\pm$1.1) }\end{tabular}

% & \begin{tabular}[c]{@{}c@{}}{ 16.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 28.9 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 37.3 }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 46.1 }\end{tabular}
\\
\multirow{1}{*}{\textbf{~~$+$SDOCL}}
% & \begin{tabular}[c]{@{}c@{}}\textrm{ SDOCL }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {33.4}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {39.5}\,($\pm$0.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {51.3}\,($\pm$0.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {57.5}\,($\pm$0.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {41.6}\,($\pm$0.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {57.5}\,($\pm$3.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {31.2}\,($\pm$0.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {49.6}\,($\pm$2.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {35.5}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ {52.6}\,($\pm$2.5) }\end{tabular}


\\
\bottomrule

\end{tabular}
}
\label{tbl:overall_comparison_biased_unbiased_setup}
\vspace{-1em}
\end{table*}


==> figures/performance_dualprompt_woste.tex <==
% \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \newcommand\fixup{\kern-\fontcharic\scriptfont2`\"}
% \bgroup
\def\arraystretch{1.0}% make the row margin compact
\begin{table}[t]
% \small
% \scriptsize
\tiny
\centering
\caption{Performance of DropTop on top of DualPrompt.}
% The highest values are marked in bold. 
% \vspace*{-0.2cm}
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
{@{}C{0.2}|C{0.2cm}C{0.2cm}C{0.2cm}|C{0.2cm}C{0.2cm}C{0.2cm}|C{0.2cm}C{0.2cm}C{0.2cm}c@{}}
% {@{}c|c|ccccccccc@{}}
\toprule
% \multicolumn{1}{c|}{} & \multicolumn{2}{c}{\textbf{\underline{    Biased Setup   }}} & \multicolumn{4}{c}{\textbf{\underline{    Unbiased Setup   }}} \\
\multicolumn{1}{c|}{\textbf{Debias}\hspace{-0.2cm}} & \multicolumn{3}{c}{\textbf{ImageNet-9}} & \multicolumn{3}{c}{\textbf{ImageNet-OnlyFG}} & \multicolumn{3}{c}{\textbf{ImageNet-Stylized}} \\
% \smallskip
\multicolumn{1}{c|}{\textbf{Method\hspace{-0.2cm}}}
& \multicolumn{1}{c}{\hspace{-0.07cm}\scalebox{.7}{\bm{$A_{avg}$}}} %{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c}{\hspace{-0.07cm}\scalebox{.7}{\bm{$A_{last}$}}}%{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c|}{\hspace{-0.07cm}\scalebox{.7}{\bm{$F_{last}$}}}%{avg} % \bm{$F_{last}$
& \multicolumn{1}{c}{\hspace{-0.07cm}\scalebox{.7}{\bm{$A_{avg}$}}}%{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c}{\hspace{-0.07cm}\scalebox{.7}{\bm{$A_{last}$}}}%{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c|}{\hspace{-0.07cm}\scalebox{.7}{\bm{$F_{last}$}}}%{avg} % \bm{$F_{last}$
& \multicolumn{1}{c}{\hspace{-0.07cm}\scalebox{.7}{\bm{$A_{avg}$}}}%{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c}{\hspace{-0.07cm}\scalebox{.7}{\bm{$A_{last}$}}}%{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c}{\hspace{-0.07cm}\scalebox{.7}{\bm{$F_{last}$}}}%{avg} % \bm{$F_{last}$
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c}{\bm{$A_{avg}$}}
\\ \toprule
% # ER ###############################################################
% \multirow{3}{*}{}
% {ER~\cite{rolnick2019experience}\!\!\hspace{-0.12cm}} 
\begin{tabular}[c]{@{}c@{}}\textrm{\hspace{0.2cm}-- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{32.8} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{45.0} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{39.3} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{49.7} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{32.8} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{45.0} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{39.3} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{49.7} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{49.7} }\end{tabular}
\\
 \begin{tabular}[c]{@{}c@{}}\textrm{\hspace{0.2cm}\algname{}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{35.9} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{47.8} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{41.3} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{38.9} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{32.8} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{45.0} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{39.3} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{49.7} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{49.7} }\end{tabular}
\\
\addlinespace[0.15ex]\cline{1-10}\addlinespace[0.6ex]
 \begin{tabular}[c]{@{}c@{}}\textrm{\hspace{0.07cm}{Rel. Improv.}\!\!\!\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}9.4\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}-6.2\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}5.1\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}21.8\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{32.8} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{45.0} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{39.3} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{49.7} }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{49.7} }\end{tabular}
\\
\bottomrule
\end{tabular}
\label{tbl:perf_dualprompt}
\end{table}

% \midrule
% # ER ###############################################################


% % DER ++ ###############################################################
% \multirow{3}{*}{DER++~\cite{buzzega2020dark}\hspace{-0.4cm}}                                                         
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{33.2}\,($\pm$0.5)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{61.6}\,($\pm$2.1) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{37.8}\,($\pm$0.7)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{60.3}\,($\pm$3.2)\!\! }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{34.5}\,($\pm$0.7)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{54.9}\,($\pm$3.2) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{39.7}\,($\pm$0.4)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{58.9}\,($\pm$4.1)\!\! }\end{tabular}
% \\
% \addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 3.7\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 11.0\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 4.9\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 2.4\% }\end{tabular}
% \\
% \midrule
% % % # ++ ###############################################################

% % # MIR ################################################################
% \multirow{3}{*}{MIR~\cite{mir}\!\!\hspace{-0.12cm}}                                               
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{32.1}\,($\pm$0.4)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{38.9}\,($\pm$3.1) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{34.0}\,($\pm$1.0)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{40.7}\,($\pm$1.6)\!\! }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{35.4}\,($\pm$1.4)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{36.0}\,($\pm$3.1) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{36.1}\,($\pm$0.6)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{38.3}\,($\pm$3.4)\!\! }\end{tabular}
% \\
% \addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 10.4\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 7.5\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 6.0\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 6.0\% }\end{tabular}
% \\
% \midrule
% % # GSS ################################################################
% \multirow{3}{*}{GSS~\cite{aljundi2019gradient}\!\!\hspace{-0.12cm}}                                               
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{34.5}\,($\pm$0.9)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{65.6}\,($\pm$0.7) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{35.3}\,($\pm$0.7)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{64.2}\,($\pm$1.9)\!\! }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{36.5}\,($\pm$0.7)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{61.6}\,($\pm$1.8) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{35.9}\,($\pm$0.4)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{62.3}\,($\pm$2.3)\!\! }\end{tabular}
% \\
% \addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 5.9\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 6.1\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 1.8\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 2.9\% }\end{tabular}
% \\
% \midrule
% % # ASER ################################################################
% \multirow{3}{*}{ASER~\cite{shim2021online}\!\!\hspace{-0.2cm}}                                               
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{30.2}\,($\pm$0.2)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{60.2}\,($\pm$0.9) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{33.6}\,($\pm$0.5)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}{56.8}\,($\pm$1.1)\!\! }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{31.2}\,($\pm$0.3)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{49.6}\,($\pm$2.8) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{35.5}\,($\pm$0.4)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.07cm}\textbf{52.6}\,($\pm$2.5)\!\! }\end{tabular}
% \\
% \addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 3.4\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 17.7\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 5.7\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 7.3\% }\end{tabular}
% \\
% \bottomrule
% \end{tabular}
% \label{tbl:perf_dualprompt}
% \end{table}


==> figures/performance_dualprompt_wste.tex <==
% \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
% \newcommand\fixup{\kern-\fontcharic\scriptfont2`\"}
% \bgroup
\def\arraystretch{1.0}% make the row margin compact
\begin{table}[t]
% \small
% \scriptsize
\tiny
\centering
\caption{Performance of DropTop on top of DualPrompt.}
% The highest values are marked in bold. 
% \vspace*{-0.3cm}
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
{@{}l|C{0.6cm}C{0.6cm}C{0.6cm}|C{0.6cm}C{0.6cm}C{0.6cm}|C{0.6cm}C{0.6cm}C{0.4cm}c@{}}
% {@{}c|c|ccccccccc@{}}
\toprule
% \multicolumn{1}{c|}{} & \multicolumn{2}{c}{\textbf{\underline{    Biased Setup   }}} & \multicolumn{4}{c}{\textbf{\underline{    Unbiased Setup   }}} \\
\multicolumn{1}{c|}{\textbf{Debias}\hspace{-0.2cm}} & \multicolumn{3}{c}{\textbf{ImageNet-9}} & \multicolumn{3}{c}{\textbf{ImageNet-OnlyFG}} & \multicolumn{3}{c}{\textbf{ImageNet-Stylized}} \\
% \smallskip
\multicolumn{1}{c|}{\textbf{Method\hspace{-0.2cm}}}
& \multicolumn{1}{c}{\scalebox{.7}{\bm{$A_{avg}$}}} %{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c}{\scalebox{.7}{\bm{$A_{avg}$}}}%{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c|}{\scalebox{.7}{\bm{$A_{avg}$}}}%{avg} % \bm{$F_{last}$
& \multicolumn{1}{c}{\scalebox{.7}{\bm{$A_{avg}$}}}%{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c}{\scalebox{.7}{\bm{$A_{avg}$}}}%{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c|}{\scalebox{.7}{\bm{$A_{avg}$}}}%{avg} % \bm{$F_{last}$
& \multicolumn{1}{c}{\scalebox{.7}{\bm{$A_{avg}$}}}%{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c}{\scalebox{.7}{\bm{$A_{avg}$}}}%{avg} % \bm{$A_{avg}$
& \multicolumn{1}{c}{\scalebox{.7}{\bm{$A_{avg}$}}}%{avg} % \bm{$F_{last}$
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c}{\bm{$A_{avg}$}}
\\ \toprule
% # ER ###############################################################
% \multirow{3}{*}{}
% {ER~\cite{rolnick2019experience}\!\!\hspace{-0.12cm}} 
\begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{32.8}\,($\pm$0.4)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{45.0}\,($\pm$1.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{39.3}\,($\pm$0.3)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{49.7}\,($\pm$0.9)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{32.8}\,($\pm$0.4)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{45.0}\,($\pm$1.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{39.3}\,($\pm$0.3)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{49.7}\,($\pm$0.9)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{49.7}\,($\pm$0.9)\!\! }\end{tabular}
\\
 \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.9}\,($\pm$0.9)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{47.8}\,($\pm$3.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{41.3}\,($\pm$0.1)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{38.9}\,($\pm$2.6)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{32.8}\,($\pm$0.4)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{45.0}\,($\pm$1.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{39.3}\,($\pm$0.3)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{49.7}\,($\pm$0.9)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{49.7}\,($\pm$0.9)\!\! }\end{tabular}
\\
\addlinespace[0.15ex]\cline{1-10}\addlinespace[0.6ex]
 \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 9.4\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ -6.2\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 5.1\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 21.8\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{32.8}\,($\pm$0.4)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{45.0}\,($\pm$1.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{39.3}\,($\pm$0.3)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{49.7}\,($\pm$0.9)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{49.7}\,($\pm$0.9)\!\! }\end{tabular}
\\
\bottomrule
\end{tabular}
\label{tbl:perf_dualprompt}
\end{table}

% \midrule
% # ER ###############################################################


% % DER ++ ###############################################################
% \multirow{3}{*}{DER++~\cite{buzzega2020dark}\hspace{-0.4cm}}                                                         
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{33.2}\,($\pm$0.5)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{61.6}\,($\pm$2.1) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{37.8}\,($\pm$0.7)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{60.3}\,($\pm$3.2)\!\! }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{34.5}\,($\pm$0.7)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{54.9}\,($\pm$3.2) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{39.7}\,($\pm$0.4)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{58.9}\,($\pm$4.1)\!\! }\end{tabular}
% \\
% \addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 3.7\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 11.0\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 4.9\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 2.4\% }\end{tabular}
% \\
% \midrule
% % % # ++ ###############################################################

% % # MIR ################################################################
% \multirow{3}{*}{MIR~\cite{mir}\!\!\hspace{-0.12cm}}                                               
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{32.1}\,($\pm$0.4)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{38.9}\,($\pm$3.1) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{34.0}\,($\pm$1.0)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{40.7}\,($\pm$1.6)\!\! }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.4}\,($\pm$1.4)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{36.0}\,($\pm$3.1) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{36.1}\,($\pm$0.6)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{38.3}\,($\pm$3.4)\!\! }\end{tabular}
% \\
% \addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 10.4\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 7.5\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 6.0\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 6.0\% }\end{tabular}
% \\
% \midrule
% % # GSS ################################################################
% \multirow{3}{*}{GSS~\cite{aljundi2019gradient}\!\!\hspace{-0.12cm}}                                               
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{34.5}\,($\pm$0.9)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{65.6}\,($\pm$0.7) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{35.3}\,($\pm$0.7)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{64.2}\,($\pm$1.9)\!\! }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{36.5}\,($\pm$0.7)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{61.6}\,($\pm$1.8) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.9}\,($\pm$0.4)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{62.3}\,($\pm$2.3)\!\! }\end{tabular}
% \\
% \addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 5.9\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 6.1\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 1.8\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 2.9\% }\end{tabular}
% \\
% \midrule
% % # ASER ################################################################
% \multirow{3}{*}{ASER~\cite{shim2021online}\!\!\hspace{-0.2cm}}                                               
% & \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{30.2}\,($\pm$0.2)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{60.2}\,($\pm$0.9) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{33.6}\,($\pm$0.5)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{56.8}\,($\pm$1.1)\!\! }\end{tabular}
% \\
% & \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{31.2}\,($\pm$0.3)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{49.6}\,($\pm$2.8) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.5}\,($\pm$0.4)\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{52.6}\,($\pm$2.5)\!\! }\end{tabular}
% \\
% \addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
% & \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 3.4\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 17.7\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 5.7\% }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ 7.3\% }\end{tabular}
% \\
% \bottomrule
% \end{tabular}
% \label{tbl:perf_dualprompt}
% \end{table}


==> figures/performance_unbiased_setup.tex <==
% \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand\fixup{\kern-\fontcharic\scriptfont2`\"}
% \bgroup
\def\arraystretch{1.2}% make the row margin compact
\begin{table}[t]
% \small
\scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
\caption{Average accuracy\,(higher is better) and forgetting\,(lower is better) on Split ImageNet-OnlyFG and Split ImageNet-Stylized for unbiased setup. The highest values are marked in bold. }
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
{@{}l|c||C{0.9cm}C{1.0cm}|C{0.9cm}C{1.0cm}c@{}}
% {@{}c|c|ccccccccc@{}}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{1}{c||}{} & \multicolumn{4}{c}{\textbf{\underline{    Unbiased Setup   }}} \\
\multicolumn{1}{c|}{\textbf{OCL}} & \multicolumn{1}{c||}{\textbf{Debias}\hspace{-0.2cm}} & \multicolumn{2}{c}{\textbf{ImageNet-OnlyFG}} & \multicolumn{2}{c}{\textbf{ImageNet-Stylized}} \\
% \smallskip
\multicolumn{1}{c|}{\textbf{Method}}
& \multicolumn{1}{c||}{\textbf{Method\hspace{-0.2cm}}}
& \multicolumn{1}{c}{\bm{$A_{avg}$}{\,($\uparrow\fixup$)}}
& \multicolumn{1}{c|}{\bm{$F_{last}$}{\,($\downarrow$)}}
& \multicolumn{1}{c}{\bm{$A_{avg}$}{\,($\uparrow\fixup$)}}
& \multicolumn{1}{c}{\bm{$F_{last}$}{\,($\downarrow$)}}
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c}{\bm{$A_{avg}$}}
\\ \toprule
% # ER ###############################################################
\multirow{2}{*}{ER~\cite{rolnick2019experience}\hspace{-0.12cm}}                                
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 39.89 }\,($\pm$2.35) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 55.36 }\,($\pm$0.30) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 19.22 }\,($\pm$0.25) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 25.34 }\,($\pm$0.18) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {50.95}\,($\pm$2.14) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {44.48}\,($\pm$1.38) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{32.8}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{45.0}\,($\pm$1.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{39.3}\,($\pm$0.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{49.7}\,($\pm$0.9) }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{SDOCL\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 37.60 }\,($\pm$1.89) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 61.02 }\,($\pm$0.61) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 18.28 }\,($\pm$1.31) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 26.45 }\,($\pm$0.17) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {36.12}\,($\pm$4.74) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {48.94}\,($\pm$1.01) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.9}\,($\pm$0.9) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{47.8}\,($\pm$3.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{41.3}\,($\pm$0.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{38.9}\,($\pm$2.6) }\end{tabular}
\\
\midrule
% # ER ###############################################################


% DER ++ ###############################################################
\multirow{2}{*}{DER++~\cite{buzzega2020dark}\hspace{-0.12cm}}                                                         
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 28.20 }\,($\pm$1.48) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 59.76 }\,($\pm$0.76) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 33.43 }\,($\pm$0.73) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 23.64 }\,($\pm$0.32) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {63.0}\,($\pm$4.62) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {44.2}\,($\pm$1.01) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{33.2}\,($\pm$0.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{61.6}\,($\pm$2.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{37.8}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{60.3}\,($\pm$3.2) }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{SDOCL\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 23.68 }\,($\pm$0.98) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 62.56 }\,($\pm$0.73) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 31.11 }\,($\pm$1.15) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 25.14 }\,($\pm$0.27) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {60.73}\,($\pm$5.06) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {45.42}\,($\pm$0.54) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{34.5}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{54.9}\,($\pm$3.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{39.7}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{58.9}\,($\pm$4.1) }\end{tabular}
\\
\midrule
% % # ++ ###############################################################

% # MIR ################################################################
\multirow{2}{*}{MIR~\cite{mir}\hspace{-0.12cm}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {58.42}\,($\pm$1.28) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {51.54}\,($\pm$0.5) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {25.32}\,($\pm$1.69) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {20.75}\,($\pm$0.56) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {41.07}\,($\pm$1.99) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {39.34}\,($\pm$1.18) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{32.1}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{38.9}\,($\pm$3.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{34.0}\,($\pm$1.0) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{40.7}\,($\pm$1.6) }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{SDOCL\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {56.25}\,($\pm$1.58) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {51.63}\,($\pm$0.56) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {25.06}\,($\pm$1.05) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {21.72}\,($\pm$0.34) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {39.25}\,($\pm$4.47) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {42.01}\,($\pm$0.93) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.4}\,($\pm$1.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{36.0}\,($\pm$3.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{36.1}\,($\pm$0.6) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{38.3}\,($\pm$3.4) }\end{tabular}
\\
\midrule
% # GSS ################################################################
\multirow{2}{*}{GSS~\cite{aljundi2019gradient}\hspace{-0.12cm}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {69.66}\,($\pm$0.71) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {46.04}\,($\pm$0.42) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {24.22}\,($\pm$0.73) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {20.95}\,($\pm$0.37) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {71.53}\,($\pm$2.01) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {40.33}\,($\pm$0.63) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{34.5}\,($\pm$0.9) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{65.6}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{35.3}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{64.2}\,($\pm$1.9) }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{SDOCL\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {69.22}\,($\pm$1.53) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {49.05}\,($\pm$0.46) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {29.06}\,($\pm$0.87) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {24.45}\,($\pm$0.27) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {68.53}\,($\pm$1.87) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {41.26}\,($\pm$0.57) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{36.5}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{61.6}\,($\pm$1.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.9}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{62.3}\,($\pm$2.3) }\end{tabular}
\\
\midrule
% # ASER ################################################################
\multirow{2}{*}{ASER~\cite{shim2021online}\hspace{-0.12cm}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 57.77 }\,($\pm$3.33) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 50.32 }\,($\pm$0.45) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 41.77 }\,($\pm$0.41) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 32.68 }\,($\pm$0.10) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {62.63}\,($\pm$2.05) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {39.7}\,($\pm$0.72) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{30.2}\,($\pm$0.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{60.2}\,($\pm$0.9) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{33.6}\,($\pm$0.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{56.8}\,($\pm$1.1) }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{SDOCL\hspace{-0.2cm}}\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 57.54 }\,($\pm$0.75) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 51.32 }\,($\pm$0.32) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 39.54 }\,($\pm$0.81) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ { 33.43 }\,($\pm$0.38) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {57.5}\,($\pm$3.18) }\end{tabular}
% & \begin{tabular}[c]{@{}c@{}}{ {41.6}\,($\pm$0.76) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{31.2}\,($\pm$0.3) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{49.6}\,($\pm$2.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.5}\,($\pm$0.4) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{52.6}\,($\pm$2.5) }\end{tabular}
\\
\bottomrule
\end{tabular}
\label{tbl:overall_comparison_unbiased_setup}
\end{table}


==> figures/performance_unbiased_setup_improv.tex <==
% \newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand\fixup{\kern-\fontcharic\scriptfont2`\"}
% \bgroup
\def\arraystretch{1.0}% make the row margin compact
\begin{table}[t]
% \small
\scriptsize
% \small
% \label{tbl:RegionBuzComparison}
\centering
\caption{Average accuracy (the higher, the better) and forgetting (the lower, the better) on Split ImageNet-OnlyFG and Split ImageNet-Stylized for the unbiased setup. The highest values are marked in bold. }
% \vspace*{-0.3cm}
\begin{tabular}[c]
% {@{}c|c|C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.3cm}C{1.7cm}@{}}
{@{}l|c||C{0.9cm}C{0.9cm}|C{0.9cm}C{1.0cm}c@{}}
% {@{}c|c|ccccccccc@{}}
\toprule
\multicolumn{1}{c|}{} & \multicolumn{1}{c||}{} & \multicolumn{4}{c}{\textbf{\underline{    Unbiased Setup   }}} \\
\multicolumn{1}{c|}{\textbf{OCL}} & \multicolumn{1}{c||}{\textbf{Debias}\hspace{-0.2cm}} & \multicolumn{2}{c}{\textbf{ImageNet-OnlyFG}} & \multicolumn{2}{c}{\textbf{ImageNet-Stylized}} \\
% \smallskip
\multicolumn{1}{c|}{\textbf{Method}}
& \multicolumn{1}{c||}{\textbf{Method\hspace{-0.2cm}}}
& \multicolumn{1}{c}{\bm{$A_{avg}$}{\,($\uparrow\fixup$)}}
& \multicolumn{1}{c|}{\bm{$F_{last}$}{\,($\downarrow$)}}
& \multicolumn{1}{c}{\bm{$A_{avg}$}{\,($\uparrow\fixup$)}}
& \multicolumn{1}{c}{\bm{$F_{last}$}{\,($\downarrow$)}}
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c|}{\bm{$A_{avg}$}}
% & \multicolumn{1}{c}{\bm{$F_{last}$}}
% & \multicolumn{1}{c}{\bm{$A_{avg}$}}
\\ \toprule
% # ER ###############################################################
\multirow{3}{*}{ER~\cite{rolnick2019experience}\!\!\hspace{-0.12cm}}                                
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{32.8}\,($\pm$0.4)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{45.0}\,($\pm$1.5) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{39.3}\,($\pm$0.3)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{49.7}\,($\pm$0.9)\!\! }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.9}\,($\pm$0.9)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{47.8}\,($\pm$3.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{41.3}\,($\pm$0.1)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{38.9}\,($\pm$2.6)\!\! }\end{tabular}
\\
\addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
& \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 9.4\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ -6.2\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 5.1\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 21.8\% }\end{tabular}
\\
\midrule
% # ER ###############################################################


% DER ++ ###############################################################
\multirow{3}{*}{DER++~\cite{buzzega2020dark}\hspace{-0.4cm}}                                                         
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{33.2}\,($\pm$0.5)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{61.6}\,($\pm$2.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{37.8}\,($\pm$0.7)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{60.3}\,($\pm$3.2)\!\! }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{34.5}\,($\pm$0.7)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{54.9}\,($\pm$3.2) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{39.7}\,($\pm$0.4)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{58.9}\,($\pm$4.1)\!\! }\end{tabular}
\\
\addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
& \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 3.7\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 11.0\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 4.9\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 2.4\% }\end{tabular}
\\
\midrule
% % # ++ ###############################################################

% # MIR ################################################################
\multirow{3}{*}{MIR~\cite{mir}\!\!\hspace{-0.12cm}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{32.1}\,($\pm$0.4)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{38.9}\,($\pm$3.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{34.0}\,($\pm$1.0)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{40.7}\,($\pm$1.6)\!\! }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.4}\,($\pm$1.4)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{36.0}\,($\pm$3.1) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{36.1}\,($\pm$0.6)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{38.3}\,($\pm$3.4)\!\! }\end{tabular}
\\
\addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
& \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 10.4\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 7.5\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 6.0\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 6.0\% }\end{tabular}
\\
\midrule
% # GSS ################################################################
\multirow{3}{*}{GSS~\cite{aljundi2019gradient}\!\!\hspace{-0.12cm}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{34.5}\,($\pm$0.9)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{65.6}\,($\pm$0.7) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{35.3}\,($\pm$0.7)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{64.2}\,($\pm$1.9)\!\! }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{36.5}\,($\pm$0.7)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{61.6}\,($\pm$1.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.9}\,($\pm$0.4)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{62.3}\,($\pm$2.3)\!\! }\end{tabular}
\\
\addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
& \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 5.9\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 6.1\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 1.8\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 2.9\% }\end{tabular}
\\
\midrule
% # ASER ################################################################
\multirow{3}{*}{ASER~\cite{shim2021online}\!\!\hspace{-0.2cm}}                                               
& \begin{tabular}[c]{@{}c@{}}\textrm{ -- }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{30.2}\,($\pm$0.2)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{60.2}\,($\pm$0.9) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{33.6}\,($\pm$0.5)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}{56.8}\,($\pm$1.1)\!\! }\end{tabular}
\\
& \begin{tabular}[c]{@{}c@{}}\textrm{\algname{}\hspace{-0.2cm}}\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{31.2}\,($\pm$0.3)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{49.6}\,($\pm$2.8) }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{35.5}\,($\pm$0.4)\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{\hspace{-0.08cm}\textbf{52.6}\,($\pm$2.5)\!\! }\end{tabular}
\\
\addlinespace[0.15ex]\cline{2-6}\addlinespace[0.6ex]
& \begin{tabular}[c]{@{}c@{}}\textrm{ \!\!\!\!\!\!{Rel. Improv.}\!\!\!\!\! }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 3.4\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 17.7\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 5.7\% }\end{tabular}
& \begin{tabular}[c]{@{}c@{}}{ 7.3\% }\end{tabular}
\\
\bottomrule
\end{tabular}
\label{tbl:overall_comparison_unbiased_setup}
\end{table}

